Direct control of the small-scale energy balance in 2D fluid dynamics

We explore the direct modification of the pseudo-spectral truncation of 2D, incompressible fluid dynamics to maintain a prescribed kinetic energy spectrum. The method provides a means of simulating fluid states with defined spectral properties, for the purpose of matching simulation statistics to given information, arising from observations, theoretical prediction or high fidelity simulation. In the scheme outlined here, Nos\'e-Hoover thermostats, commonly used in molecular dynamics, are introduced as feedback controls applied to energy shells of the Fourier-discretized Navier-Stokes equations. As we demonstrate in numerical experiments, the dynamical properties (quantified using autocorrelation functions) are only modestly perturbed by our device, while ensemble dispersion is significantly enhanced in comparison with simulations of a corresponding truncation incorporating hyperviscosity.

==> comp.tex <==
25c25
< When quantifying statistical uncertainty in approximate solutions of dynamical systems, it is common to treat numerical truncation errors as random variables \cite{Evensen:09}. Such an assumption is frequently necessary to make theoretical progress. However, as demonstrated using backward error analysis \cite{HaLuWa:06}, the truncated terms can often be interpreted as correction terms linking the output of a numerical process to a higher order approximation of a modified dynamical system. Hence numerical truncation errors behave not as random variables but as deterministic perturbations that induce bias in the statistics of simulation data. 
---
> When quantifying statistical uncertainty in approximate solutions of dynamical systems, it is common to treat numerical truncation errors as random variables \cite{Evensen:09}. Such an assumption is frequently necessary to make theoretical progress. However, as demonstrated using backward error analysis \cite{HaLuWa:06,Leimkuhler:04}, the truncated terms can often be interpreted as correction terms linking the output of a numerical process to a higher order approximation of a modified dynamical system. Hence numerical truncation errors behave not as random variables but as deterministic perturbations that induce bias in the statistics of simulation data. 
34c34
< For fixed-wavelength stationary forcing and viscous dissipation, real forced fluids in the atmosphere are believed to sample a nonequilibrium steady state (NESS) in which the kinetic energy spectrum satisfies a power law as predicted by Kolmogorov \cite{TuSm06}.  In this case no equilibrium measure is explicitly known, but a stationary expectation, namely a power-law spectrum for kinetic energy can be observed, e.g.~in airplane data \cite{Nastrom:84}.
---
> For fixed-wavelength stationary forcing and viscous dissipation, real forced fluids in the atmosphere are believed to sample a nonequilibrium steady state (NESS) in which the kinetic energy spectrum satisfies a power law  over a range of length scales as predicted by Kolmogorov \cite{TuSm06}.  In this case no equilibrium measure is explicitly known, but a stationary expectation, namely the power-law spectrum for kinetic energy, can be observed, for example, in airplane data \cite{Nastrom:84}.  
36,37c36,37
< Power-law kinetic energy spectra can be simulated using forced Navier-Stokes discretizations at operational resolutions, but typically require a viscosity parameter that far exceeds that encountered in atmosphere/ocean science applications in nature.  Excessive numerical viscosity is believed to adversely affect the simulated growth of small-scale physical instabilities as well as the variance of ensemble simulations.  Turbulent back-scatter methods have been introduced in \cite{Shutts:05} to re-inject kinetic energy 
< In this paper we propose a method for enforcing a power law spectrum as observed from measurements.  Our approach allows us to maintain a given mean spectrum without a viscosity model.
---
> Power-law kinetic energy spectra can be simulated using forced Navier-Stokes discretizations at operational resolutions, but typically require a viscosity parameter that far exceeds that encountered in atmosphere/ocean science applications in nature.  Excessive numerical viscosity is believed to adversely affect the simulated growth of small-scale physical instabilities as well as the variance of ensemble simulations.  Turbulent back-scatter methods have been introduced in \cite{Shutts:05,Berner:09} to re-inject kinetic energy at viscous length scales.
> In this paper we propose a method for enforcing a power law spectrum as observed from measurements.  Our approach allows us to maintain a given mean spectrum without a viscosity model. The energy spectrum we impose can be taken from real world observations. In the case of atmospheric turbulence the experiments by \cite{NaGa:85} provide such data. In two-dimensional forced-dissipated Navier-Stokes it may also be taken from the theoretical prediction of KLB-theory.
39d38
< \noindent\rule{\textwidth}{.1pt}
43,54c42,48
< In numerical simulations, accurate solution trajectories on a short time scale do not guarantee correct long time averages of simulation observables. Errors in statistical averages may be a consequence of incorrect parameterization, or numerical bias. Well-established work on backward error analysis \cite{HaLuWa:06,Leimkuhler:04} adopts the viewpoint that the global behavior of a long numerical simulation can best be understood not as the approximation of particular trajectory but rather as an accurate sample from a perturbed continuum process described by modified equations. This implies simulation statistics are biased towards those of the modified equations. For example, in the setting of geophysical fluid dynamics, the discrete conservation laws in different discretizations of the quasi-geostrophic potential vorticity equation strongly influence the long time mean potential vorticity field and pointwise fluctuation statistics \citep{DuFr:07,Dubinkina:10}.
< 
< In the case of two-dimensional fluid dynamics there are several known equilibrium models. For unforced, inviscid, two-dimensional ideal fluids, entropy maximization with constraints due to (infinitely many) conserved quantities yields the well-established Miller/Robert-Sommeria measure \citep{Sommeria:11}. In fluctuating hydrodynamics the stochastic forcing is defined to satisfy a fluctuation-dissipation relation with respect to viscous dissipation such that the Boltzmann-Gibbs distribution is ergodic. Two-dimenional fluid flows with dissipation at small and large scales and forcing at an intermediate scale attain a non-equilibrium steady state (NESS) in which the kinetic energy spectrum satisfies a power law over a range of length scales. In this case the equilibrium measure is unknown, but the observed kinetic energy spectrum provides certain known expectations with regard to the unknown measure.
< 
< When simulating flows of this third kind, kinetic energy spectra may be found using discretized Navier-Stokes equations. But this typically requires viscosity at unnaturally large scales. This adversely affects the growth of small-scale physcial instabilities and the variance of ensemble simulations \citep{Shutts:05}. 
< 
< We propose a method for enforcing a power law energy spectrum. The energy spectrum we impose can be taken from real world observations. In the case of atmospheric turbulence the experiments by \citet{NaGa:85} provide such data. In two-dimensional forced-dissipated Navier-Stokes it may also be taken from the theoretical prediction of KLB-theory.
< 
< \noindent\rule{\textwidth}{.1pt}
< 
< 
< When simulating atmospheric flows the large range of length scales prevents resolving small scale dynamics. These scales, however, play a crucial role in the behaviour of the atmospheric dynamics. In the present work we will focus on the effect of small scale dynamics on the statistical behaviour of the large scale flow. Of particular interest is the kinetic energy spectrum that is ubiquotously observed in the atmosphere. To allow a simpler and clearer analysis, we consider two-dimensional, incompressible flow as a model for atmospheric turbulence. Whether the kinetic energy spectrum observed in the atmosphere is a case of two-dimensional turbulence or not is an open question. It is addressed in detail by \citet{Lindborg:99}. We shall not further discuss this issue here, but simply use two-dimensional turbulence as a model where small-scale dissipation plays an important role in establishing a kinetic energy spectrum.
---
> %In numerical simulations, accurate solution trajectories on a short time scale do not guarantee correct long time averages of simulation observables. Errors in statistical averages may be a consequence of incorrect parameterization, or numerical bias. Well-established work on backward error analysis \cite{HaLuWa:06,Leimkuhler:04} adopts the viewpoint that the global behavior of a long numerical simulation can best be understood not as the approximation of particular trajectory but rather as an accurate sample from a perturbed continuum process described by modified equations. This implies simulation statistics are biased towards those of the modified equations. For example, in the setting of geophysical fluid dynamics, the discrete conservation laws in different discretizations of the quasi-geostrophic potential vorticity equation strongly influence the long time mean potential vorticity field and pointwise fluctuation statistics \citep{DuFr:07,Dubinkina:10}.
> %
> %In the case of two-dimensional fluid dynamics there are several known equilibrium models. For unforced, inviscid, two-dimensional ideal fluids, entropy maximization with constraints due to (infinitely many) conserved quantities yields the well-established Miller/Robert-Sommeria measure \citep{Sommeria:11}. In fluctuating hydrodynamics the stochastic forcing is defined to satisfy a fluctuation-dissipation relation with respect to viscous dissipation such that the Boltzmann-Gibbs distribution is ergodic. Two-dimenional fluid flows with dissipation at small and large scales and forcing at an intermediate scale attain a non-equilibrium steady state (NESS) in which the kinetic energy spectrum satisfies a power law over a range of length scales. In this case the equilibrium measure is unknown, but the observed kinetic energy spectrum provides certain known expectations with regard to the unknown measure.
> %
> %When simulating flows of this third kind, kinetic energy spectra may be found using discretized Navier-Stokes equations. But this typically requires viscosity at unnaturally large scales. This adversely affects the growth of small-scale physcial instabilities and the variance of ensemble simulations \citep{Shutts:05}. 
> %
> %We propose a method for enforcing a power law energy spectrum. The energy spectrum we impose can be taken from real world observations. In the case of atmospheric turbulence the experiments by \cite{NaGa:85} provide such data. In two-dimensional forced-dissipated Navier-Stokes it may also be taken from the theoretical prediction of KLB-theory.
57c51
< When simulating atmospheric flows the large range of length scales prevents resolving small scale dynamics exactly. These small scale dynamics however play an important role in dissipating energy, for it is at these scales that viscosity acts. If these scales are unresolved the absence of dissipation is commonly compensated for by introducing other, artificial, forms of energy dissipation. These inhibit the growth of small scale instabilities and disturb the simulation at length scales that are of practical interest. Furthermore when simulating using an ensemble of initial conditions the solutions will remain too close together as a result of the lack of energy at small scales. \citep{Shutts:05} For these reasons it is desirable to divine other ways to manage the (small-scale) energy balance in atmospheric flow simulations.
---
> %When simulating atmospheric flows the large range of length scales prevents resolving small scale dynamics. These scales, however, play a crucial role in the behaviour of the atmospheric dynamics. In the present work we will focus on the effect of small scale dynamics on the statistical behaviour of the large scale flow. Of particular interest is the kinetic energy spectrum that is ubiquitously observed in the atmosphere. To allow a simpler and clearer analysis, we consider two-dimensional, incompressible flow as a model for atmospheric turbulence. 
59c53
< To avoid many of the intricacies of atmospheric fluid flow, in this paper we will focus on two-dimensioal turbulence with forcing and dissipation as a model. This combination of Hamiltonian dynamics with forcing and dissipation is similar to that of thermostated molecular dynamics. This motivates us to seek methods from molecular dynamics and apply them heuristically to turbulent fluid flow. These methods focus on statisical properties of resolved modes rather than using physical properties of the unresolved scales as is commonplace in turbulence modeling.
---
> %When simulating atmospheric flows the large range of length scales prevents resolving small scale dynamics exactly. These small scale dynamics however play an important role in dissipating energy, for it is at these scales that viscosity acts. If these scales are unresolved the absence of dissipation is commonly compensated for by introducing other, artificial, forms of energy dissipation. These inhibit the growth of small scale instabilities and disturb the simulation at length scales that are of practical interest. Furthermore when simulating using an ensemble of initial conditions the solutions will remain too close together as a result of the lack of energy at small scales. \citep{Shutts:05} For these reasons it is desirable to divine other ways to manage the (small-scale) energy balance in atmospheric flow simulations.
60a55
> %To avoid many of the intricacies of atmospheric fluid flow, in this paper we will focus on two-dimensional turbulence with forcing and dissipation as a model. This combination of Hamiltonian dynamics with forcing and dissipation is similar to that of thermostated molecular dynamics. This motivates us to seek methods from molecular dynamics and apply them heuristically to turbulent fluid flow. These methods focus on statisical properties of resolved modes rather than using physical properties of the unresolved scales as is commonplace in turbulence modeling.
64c59,61
< We shall use the two-dimensional, incompressible Navier-Stokes equations on a periodic domain as a model for atmospheric fluid flow. An incompressible flow field is uniquely determined by its stream function $\psi$ via $u = -\partial_y \psi$ and $v = \partial_x \psi$. The vorticity $\omega = \Delta \psi$ is the Laplacian of the stream function, it is convenient to write the dynamics in terms of the vorticity:
---
> To avoid many of the intricacies of geophysical fluid flows, we will focus on driven two-dimensional incompressible flow with Ekman drag and linear viscosity. We ignore the effects of rotation and topography, and work with the Navier-Stokes equations on a doubly periodic domain.  Whether the kinetic energy spectrum observed in the atmosphere is a case of two-dimensional turbulence or not is an open question \cite{Lindborg:99}. We shall not further discuss this issue here, but simply use ``two-dimensional turbulence'' as a model where small-scale dissipation plays an important role in establishing a kinetic energy spectrum.
> 
> A 2D incompressible flow field is uniquely determined by its stream function $\psi$ via $u = -\partial_y \psi$ and $v = \partial_x \psi$. The vorticity $\omega = \Delta \psi$ is the Laplacian of the stream function, it is convenient to write the dynamics in terms of the vorticity:
84c81,82
< where $J_{\bs{k}}(\bs{\omega})$ is  the operator of \eqref{eq:J} in spectral form. This nonlinear term is numerically evaluated on a physical grid. A two-thirds de-aliasing filter is used in all simulations in this work. In a more practical application it may be better to suffer aliasing for the benefit of higher spatial resolution at the same computational expense. \citet[Ch. 11]{Boyd:13}
---
> where $J_{\bs{k}}(\bs{\omega})$ is  the operator of \eqref{eq:J} in spectral form. This nonlinear term is numerically evaluated on a physical grid. A two-thirds de-aliasing filter is used in all simulations in this work \cite{Canuto:06}. 
> %In a more practical application it may be better to suffer aliasing for the benefit of higher spatial resolution at the same computational expense. \cite[Ch. 11]{Boyd:13}
86c84
< In this study we use a set-up similar to that of \citet{Gotoh:98}, i.e. the dissipation is limited to a viscous term, $p=1$, and a hypoviscous term with $p=-1$ in order to curtail the inverse energy cascade. This term is analogous to bottom friction in atmospheric fluid flow. \citep{DaGu:00} The effect of the hypoviscosity is restricted to those modes with $|\bs{k}| \leq 3$. The forcing is Gaussian white noise in time and in Fourier space. Only modes with wavenumber magnitude in the range $4 \leq |\bs{k}| \leq 6$ are forced. The magnitude of the forcing is scaled such that the expected power input matches a given value $P$, the forcing is described in detail in Appendix \ref{sec:forcing}. The values of the parameters used in various simulations are summarized in Table \ref{tab:pars}.
---
> In this study we use a set-up similar to that of \cite{Gotoh:98}, i.e. the dissipation is limited to a viscous term, $p=1$, and a hypoviscous term with $p=-1$ in order to curtail the inverse energy cascade. This term is analogous to bottom friction in atmospheric fluid flow. \citep{DaGu:00} The effect of the hypoviscosity is restricted to those modes with $|\bs{k}| \leq 3$. The forcing is Gaussian white noise in time and in Fourier space. Only modes with wavenumber magnitude in the range $4 \leq |\bs{k}| \leq 6$ are forced. The magnitude of the forcing is scaled such that the expected power input matches a given value $P$, the forcing is described in detail in Appendix \ref{sec:forcing}. The values of the parameters used in various simulations are summarized in Table \ref{tab:pars}.
117c115
< The hypo- and hyperdiffusion terms in the turbulence equations have typical length scales defined by the wave number magnitude for which the coefficient $\nu_p \Delta_{\bs{k}}^p$ has magnitude unity. By using $\Delta_{\bs{k}} = -|\bs{k}|^2$ we find $k_d = \sqrt{\nu_1}^{-1}$ for $p=1$ and $k_h = \sqrt{\nu_{-1}}$ for $p=-1$. Assume that these two scales are sufficiently separated and that the forcing acts primarily at some intermediate length scale. In this setting it is expected that the hypothesis of \citet{Kraichnan:67} holds, and that there is a flux with constant energy from the forced scales to larger scales, and a flux with constant enstrophy to smaller scales. These fluxes will terminate when the dissipative scales $k_h$ and $k_d$ are reached, but with sufficient separation between forcing and dissipation scales there will still be regions of constant energy and enstrophy transport. Because these ranges exist in the absence of damping and forcing, they are dubbed inertial ranges. The transport of 
---
> The hypo- and hyperdiffusion terms in the turbulence equations have typical length scales defined by the wave number magnitude for which the coefficient $\nu_p \Delta_{\bs{k}}^p$ has magnitude unity. By using $\Delta_{\bs{k}} = -|\bs{k}|^2$ we find $k_d = \sqrt{\nu_1}^{-1}$ for $p=1$ and $k_h = \sqrt{\nu_{-1}}$ for $p=-1$. Assume that these two scales are sufficiently separated and that the forcing acts primarily at some intermediate length scale. In this setting it is expected that the hypothesis of \cite{Kraichnan:67} holds, and that there is a flux with constant energy from the forced scales to larger scales, and a flux with constant enstrophy to smaller scales. These fluxes will terminate when the dissipative scales $k_h$ and $k_d$ are reached, but with sufficient separation between forcing and dissipation scales there will still be regions of constant energy and enstrophy transport. Because these ranges exist in the absence of damping and forcing, they are dubbed inertial ranges. The transport of 
142c140
< The energy spectrum in these results appears steeper than the hypothesized $k^{-3}$ slope. This is common in numerical simulations and is usually attributed to insufficiently large Reynolds number due to limited resolution\footnote{\citet{Saffman:71} suggests a $k^{-4}$ spectrum as the result of small discontinuities at the smallest scales.}. \citep{Bofetta:10,Gotoh:98,BrMcMuPrWe:00} Therefore we follow \citet{Gotoh:98} in trying to find a relationship of the form
---
> The energy spectrum in these results appears steeper than the hypothesized $k^{-3}$ slope. This is common in numerical simulations and is usually attributed to insufficiently large Reynolds number due to limited resolution\footnote{\cite{Saffman:71} suggests a $k^{-4}$ spectrum as the result of small discontinuities at the smallest scales.}. \citep{Bofetta:10,Gotoh:98,BrMcMuPrWe:00} Therefore we follow \cite{Gotoh:98} in trying to find a relationship of the form
215c213
< The tendency of forced-dissipated turbulence to develop a power law spectrum that is independent of initial conditions and time step-size suggests the dynamics have a unique invariant measure and are therefore ergodic. The ergodicity of the forced-dissipated two-dimensional Navier-Stokes equations is proven by \citet{EMa:01} for the case of forcing only modes $(1,1)$ and either $(1,0)$ or $(0,1)$. Following the same techniques used therein, it is readily proven that the same result holds when there exist forced modes $\bs{k}_1$ and $\bs{k}_2$ such that both $\bs{k}_1 + (1,0)$ and $\bs{k}_2 + (0,2)$ are also forced. These results only hold for a system that has finitely many resolved modes. With finite dissipation any arbitrary accuracy may be achieved by choosing a sufficiently large, yet finite, number of modes to include in the state vector.
---
> The tendency of forced-dissipated turbulence to develop a power law spectrum that is independent of initial conditions and time step-size suggests the dynamics have a unique invariant measure and are therefore ergodic. The ergodicity of the forced-dissipated two-dimensional Navier-Stokes equations is proven by \cite{EMa:01} for the case of forcing only modes $(1,1)$ and either $(1,0)$ or $(0,1)$. Following the same techniques used therein, it is readily proven that the same result holds when there exist forced modes $\bs{k}_1$ and $\bs{k}_2$ such that both $\bs{k}_1 + (1,0)$ and $\bs{k}_2 + (0,2)$ are also forced. These results only hold for a system that has finitely many resolved modes. With finite dissipation any arbitrary accuracy may be achieved by choosing a sufficiently large, yet finite, number of modes to include in the state vector.
235c233
< In particular, let us study the energy spectrum as a set of observables. Given a truncation that is just below $k_d$, the modes $\bar\omega_{\bs{k}}$ with $|\bs{k}| >> k_f$ show a power law spectrum due to the forward enstrophy cascade. In the truncated system, this cascade of enstrophy from the one energy band to the next is halted abruptly. This yields an unphysical build-up of enstrophy at the smallest resolved scales, known as spectral blocking. Furthermore, an inaccurate energy spectrum at the smallest modes is named by \citet{SuGaCh:99} as the cause for a deviation from the power law spectrum in the energy range, i.e. in the large scales.
---
> In particular, let us study the energy spectrum as a set of observables. Given a truncation that is just below $k_d$, the modes $\bar\omega_{\bs{k}}$ with $|\bs{k}| >> k_f$ show a power law spectrum due to the forward enstrophy cascade. In the truncated system, this cascade of enstrophy from the one energy band to the next is halted abruptly. This yields an unphysical build-up of enstrophy at the smallest resolved scales, known as spectral blocking. Furthermore, an inaccurate energy spectrum at the smallest modes is named by \cite{SuGaCh:99} as the cause for a deviation from the power law spectrum in the energy range, i.e. in the large scales.
341c339
< The Fourier pseudo-spectral method used is not readily generalizable to other flow domains. On the other hand, finite volume, finite element and finite difference schemes do not in themselves give information about the spectrum of energy in wavenumber space. A compromise between the two approaches is given by wavelet methods. \citep{Meyer:95} Wavelets allow expanding the voriticity field in a manner that is local in physical space as well as in wavenumber space. \citet{FaKePeGo:96} use wavelet methods to analyse turbulent velocity fields and define a local energy spectrum. In fact they discover that the $k^{-3}$ energy spectrum only holds outside of regions of strong voricity and shear layers. Inside those regions the energy spectrum scales as $k^{-6}$ and $k^{-4}$ respectively. \citet{FrSc:99} simulate two-dimensional turbulent dynamics using a wavelet basis as the degrees of freedom. In this setting applying our control method might be even more effective, as the action can be restricted to the homogenous 
---
> The Fourier pseudo-spectral method used is not readily generalizable to other flow domains. On the other hand, finite volume, finite element and finite difference schemes do not in themselves give information about the spectrum of energy in wavenumber space. A compromise between the two approaches is given by wavelet methods. \citep{Meyer:95} Wavelets allow expanding the voriticity field in a manner that is local in physical space as well as in wavenumber space. \cite{FaKePeGo:96} use wavelet methods to analyse turbulent velocity fields and define a local energy spectrum. In fact they discover that the $k^{-3}$ energy spectrum only holds outside of regions of strong voricity and shear layers. Inside those regions the energy spectrum scales as $k^{-6}$ and $k^{-4}$ respectively. \cite{FrSc:99} simulate two-dimensional turbulent dynamics using a wavelet basis as the degrees of freedom. In this setting applying our control method might be even more effective, as the action can be restricted to the homogenous 
344c342
< The goal of the work by \citet{FaKePr:11} is similar to ours, to achieve a simulation with the desired power law energy spectrum. Their focus, however, is on finding forcing functions that result in the hypothesized $k^{-5/3}$ and  $k^{-3}$ power law regimes. They suggest the reason numerical simulation differ from the hypothesized spectra is not due to insufficient resolution, but due to the choice of forcing. This is in line with \citet{DaGu:00}, who demonstrate the the power law spectra can only be observed for a special set of external parameters.
---
> The goal of the work by \cite{FaKePr:11} is similar to ours, to achieve a simulation with the desired power law energy spectrum. Their focus, however, is on finding forcing functions that result in the hypothesized $k^{-5/3}$ and  $k^{-3}$ power law regimes. They suggest the reason numerical simulation differ from the hypothesized spectra is not due to insufficient resolution, but due to the choice of forcing. This is in line with \cite{DaGu:00}, who demonstrate the the power law spectra can only be observed for a special set of external parameters.


==> packages.tex <==
%
% Eingebundene Pakete
%
\usepackage[english]{babel}
\usepackage{natbib}
\usepackage[dvips]{graphicx}
%\usepackage[dvips]{color}                % Farben im Text
%\usepackage{a4wide}
%\usepackage{fancyheadings}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{rotating}
\usepackage{float}
\usepackage{psfrag}
%\usepackage{pstcol,pst-plot}
\usepackage{pstricks}
%\usepackage{lscape}
%\usepackage{dcolumn}
%\usepackage{calc}
%\usepackage[T1]{fontenc}                  % Korrekte Trennung mit Umlauten aber inkompatibel mit CM Type1-Fonts
%\usepackage{ae}                          % Korrekte Trennung mit Umlauten kompatibel mit CM Type1-Fonts
%\usepackage{aecompl}                     % Komplettierung der ae-fonts
%\usepackage[latin1]{inputenc}
%age[ps2pdf,dvips,colorlinks,urlcolor=blue,citecolor=black,linkcolor=black,bookmarks=false]{hyperref}
\usepackage{subfig}
\usepackage{paralist}
%\usepackage{nomencl}
\usepackage{syntonly}
\usepackage{ifthen}
\usepackage{array}
\usepackage{fancyhdr}
\usepackage{alltt}
\usepackage{algorithm}
\usepackage{algorithmic}
%
% Notizen:
% 
% Der Befehl \usepackage[T1]{fontenc} darf nicht in Zusammenhang mit dem Befehl
% dvips -Ppdf zum Erstellen eines Type1-Fonts enthaldenden pdf-Dokumentes benutzt
% werden. Wird das T1-Fontencoding dennoch gewlt produziert dvips bitmap fonts!
%
%
% ZE-fonts:
%
% Ein nicht ganz vollwertiger Ersatz von EC-Schriften im Type-1-Format,
% mit denen man denselben Umbruch wie mit den EC-Schriften erht,
% besteht darin, T1-kodierte virtuelle Fonts zu benutzen, die die
% Schriften der Computer-Modern-(CM)-Familie verwenden, da die
% CM-Schriftfamilie in Type-1-Format vorliegt. Solche virtuelle
% Schriften sind unter dem Namen Almost-European-(AE)-Schriften und
% unter dem Namen ZE verfgbar.

